Near-Infrared Photometry of the Type IIn SN 2005ip: The Case for Dust Condensation

Near-infrared photometric observations of the Type IIn SN 2005ip in NGC 2906 reveal large fluxes (>1.3 mJy) in the K_s-band over more than 900 days. While warm dust can explain the late-time K_s-band emission of SN 2005ip, the nature of the dust heating source is ambiguous. Shock heating of pre-existing dust by post-shocked gas is unlikely because the forward shock is moving too slowly to have traversed the expected dust-free cavity by the time observations first reveal the K_s emission. While an infrared light echo model correctly predicts a near-infrared luminosity plateau, heating dust to the observed temperatures of ~1400-1600 K at a relatively large distance from the supernova (> 10^{18} cm) requires an extraordinarily high early supernova luminosity (~1 X 10^{11} L_solar). The evidence instead favors condensing dust in the cool, dense shell between the forward and reverse shocks. Both the initial dust temperature and the evolutionary trend towards lower temperatures are consistent with this scenario. We infer that radiation from the circumstellar interaction heats the dust. While this paper includes no spectroscopic confirmation, the photometry is comparable to other SNe that do show spectroscopic evidence for dust formation. Observations of dust formation in SNe are sparse, so these results provide a rare opportunity to consider SNe Type IIn as dust sources.

==> tab1.tex <==
\tablehead{
\colhead{JD} & \colhead{Epoch} & \colhead{J} & \colhead{H} &
\colhead{K$_{\rm s}$} & \colhead{J} & \colhead{H} & \colhead{K$_{\rm s}$}\\
\colhead{(2450000+)} & \colhead{(days)} & \colhead{(mag)} & \colhead{(mag)} & \colhead{(mag)} & \colhead{(mJy)} & \colhead{(mJy)} & \colhead{(mJy)}
}
\startdata
3686.5 & 7.0 & 14.42(0.01) & - & 13.87(0.01) & 2.84(0.03) & - & 1.75(0.02) \\
3688.0 & 8.0 & 14.41(0.01) & - & 13.93(0.02) & 2.88(0.03) & - & 1.66(0.03) \\
3743.0 & 63.0 & 15.42(0.03) & 14.91(0.05) & 14.12(0.03) & 1.14(0.03) &
1.07(0.05) & 1.39(0.03) \\
3763.1 & 83.0 & 15.51(0.03) & 14.71(0.03) & 13.82(0.02) & 1.04(0.03) &
1.28(0.04) & 1.83(0.03) \\
3773.0 & 93.0 & 15.59(0.03) & 14.66(0.03) & 13.75(0.01) & 0.97(0.02) &
1.34(0.04) & 1.96(0.03) \\
3799.5 & 120.0 & 15.84(0.03) & 14.66(0.03) & 13.67(0.01) & 0.77(0.02) &
1.34(0.04) & 2.11(0.03) \\
3830.7 & 151.0 & 16.08(0.04) & 14.77(0.03) & 13.72(0.01) & 0.62(0.02) &
1.21(0.04) & 2.01(0.03) \\
3850.5 & 171.0 & 16.21(0.05) & 14.81(0.04) & 13.75(0.02) & 0.54(0.02) &
1.16(0.04) & 1.97(0.04) \\
3865.5 & 186.0 & 15.96(0.04) & 14.75(0.04) & 13.67(0.01) & 0.69(0.02) &
1.23(0.04) & 2.12(0.03) \\
3879.5 & 200.0 & 16.05(0.05) & 14.78(0.04) & 13.67(0.02) & 0.63(0.03) &
1.20(0.04) & 2.10(0.03) \\
4030.9 & 351.0 & 16.25(0.05) & - & 13.75(0.01) & 0.53(0.02) & - & 1.96(0.03) \\
4112.0 & 432.0 & 16.49(0.06) & 15.20(0.05) & 13.87(0.01) & 0.42(0.02) &
0.82(0.04) & 1.75(0.02) \\
4159.8 & 480.0 & 16.60(0.07) & 15.15(0.05) & 13.89(0.02) & 0.38(0.02) &
0.85(0.04) & 1.73(0.03) \\
4227.6 & 548.0 & 16.66(0.08) & 15.23(0.06) & 13.96(0.02) & 0.36(0.03) &
0.79(0.04) & 1.62(0.03) \\
4367.9 & 688.0 & 16.76(0.08) & 15.48(0.07) & 13.92(0.02) & 0.33(0.02) &
0.63(0.04) & 1.68(0.03) \\
4406.8 & 722.0 & 16.85(0.09) & 15.52(0.07) & 14.03(0.02) & 0.30(0.03) &
0.61(0.04) & 1.52(0.03) \\
4452.9 & 767.0 & 16.94(0.11) & 15.67(0.08) & 14.07(0.02) & 0.28(0.03) &
0.53(0.04) & 1.46(0.02) \\
4516.8 & 831.0 & - & 15.87(0.11) & 14.14(0.03) & - & 0.44(0.05) & 1.37(0.04) \\
4537.6 & 852.0 & 17.03(0.10) & 15.80(0.09) & 14.10(0.02) & 0.26(0.02) &
0.47(0.04) & 1.42(0.03) \\
4580.6 & 895.0 & 17.01(0.10) & 15.83(0.09) & 14.12(0.02) & 0.26(0.02) &
0.45(0.04) & 1.40(0.02) \\
4620.6 & 935.0 & 17.17(0.12) & 16.14(0.15) & 14.18(0.05) & 0.23(0.03) &
0.34(0.05) & 1.32(0.06)
\enddata




==> tab2.tex <==
\tablehead{
\colhead{Epoch} & \colhead{J-H} & \colhead{J-K$_{\rm s}$} & \colhead{H-K$_{\rm s}$}\\
\colhead{(days)} & \colhead{(mag)} & \colhead{(mag)} & \colhead{(mag)}
}
\startdata
7 & - & 0.55(0.02) & - \\
8 & - & 0.48(0.02) & - \\
63 & 0.51(0.06) & 1.30(0.04) & 0.78(0.06) \\
83 & 0.81(0.04) & 1.69(0.03) & 0.89(0.04) \\
93 & 0.93(0.04) & 1.85(0.03) & 0.92(0.03) \\
120 & 1.18(0.05) & 2.17(0.04) & 0.99(0.03) \\
151 & 1.31(0.06) & 2.36(0.05) & 1.05(0.04) \\
171 & 1.40(0.06) & 2.47(0.05) & 1.07(0.04) \\
186 & 1.21(0.05) & 2.30(0.04) & 1.09(0.04) \\
200 & 1.27(0.06) & 2.38(0.05) & 1.11(0.04) \\
351 & - & 2.50(0.05) & - \\
432 & 1.29(0.08) & 2.62(0.06) & 1.33(0.05) \\
480 & 1.45(0.08) & 2.72(0.07) & 1.27(0.05) \\
548 & 1.43(0.09) & 2.70(0.08) & 1.27(0.06) \\
688 & 1.29(0.11) & 2.85(0.08) & 1.56(0.07) \\
722 & 1.35(0.11) & 2.84(0.09) & 1.49(0.07) \\
767 & 1.29(0.13) & 2.89(0.11) & 1.60(0.08) \\
831 & -15.87(0.11) & -14.14(0.03) & 1.73(0.12) \\
852 & 1.24(0.14) & 2.94(0.10) & 1.70(0.09) \\
895 & 1.18(0.13) & 2.90(0.10) & 1.72(0.09) \\
935 & 1.04(0.19) & 2.99(0.13) & 1.95(0.16)
\enddata

==> tab3.tex <==
\tablehead{
\colhead{Epoch} & \colhead{T$_{bb}$} & \colhead{T$_{\lambda^{-1}}$} &
\colhead{T$_{\lambda^{-2}}$} & \colhead{L$_{bb}$} & \colhead{L$_{\lambda^{-1}}$}
& \colhead{L$_{\lambda^{-2}}$} & \colhead{L$_{\rm radioactive}$} \\
\colhead{(d)} & \colhead{(K)} & \colhead{(K)} & \colhead{(K)} &
\colhead{$(10^{41} \rm erg~s^{-1})$} & \colhead{$(10^{41} \rm erg~s^{-1})$} &
\colhead{$(10^{41} \rm erg~s^{-1})$} & \colhead{$(10^{41} \rm erg~s^{-1})$}
}
\startdata
7 & - & - & - & - & - & - & 42.09 \\
8 & - & - & - & - & - & - & 42.09 \\
63 & 1969(89) & 1547(56) & 1279(39) & 41.43(0.03) & 41.38(0.03) & 41.34(0.03) &
41.86 \\
83 & 1809(47) & 1449(31) & 1213(22) & 41.53(0.01) & 41.48(0.02) & 41.43(0.02) &
41.80 \\
93 & 1765(44) & 1422(29) & 1194(20) & 41.57(0.01) & 41.50(0.01) & 41.46(0.01) &
41.75 \\
120 & 1667(38) & 1359(26) & 1149(18) & 41.59(0.01) & 41.53(0.01) & 41.49(0.01) &
41.64 \\
151 & 1599(39) & 1314(27) & 1118(19) & 41.57(0.01) & 41.50(0.01) & 41.46(0.01) &
41.53 \\
171 & 1582(45) & 1303(31) & 1110(22) & 41.56(0.02) & 41.50(0.02) & 41.46(0.02) &
41.45 \\
186 & 1561(38) & 1289(26) & 1100(19) & 41.60(0.01) & 41.53(0.01) & 41.49(0.01) &
41.39 \\
200 & 1538(38) & 1273(26) & 1088(19) & 41.59(0.01) & 41.53(0.01) & 41.49(0.02) &
41.34 \\
351 & - & - & - & - & - & - & 40.75 \\
432 & 1345(39) & 1140(28) & 990(21) & 41.53(0.02) & 41.48(0.02) & 41.42(0.02) &
40.43 \\
480 & 1390(41) & 1172(29) & 1013(22) & 41.53(0.02) & 41.46(0.02) & 41.41(0.02) &
40.25 \\
548 & 1386(48) & 1169(34) & 1012(26) & 41.50(0.02) & 41.43(0.02) & 41.38(0.02) &
39.98 \\
688 & 1186(42) & 1024(31) & 902(24) & 41.59(0.02) & 41.50(0.02) & 41.43(0.02) &
39.43 \\
722 & 1229(45) & 1056(34) & 926(26) & 41.52(0.02) & 41.43(0.02) & 41.38(0.02) &
39.31 \\
767 & 1163(45) & 1007(33) & 888(26) & 41.53(0.02) & 41.45(0.02) & 41.39(0.02) &
39.14 \\
831 & 1093(59) & 954(45) & 847(35) & 41.55(0.03) & 41.46(0.03) & 41.39(0.04) &
38.89 \\
852 & 1108(48) & 966(36) & 856(28) & 41.56(0.03) & 41.46(0.03) & 41.39(0.03) &
38.82 \\
895 & 1098(46) & 958(35) & 850(28) & 41.56(0.02) & 41.46(0.03) & 41.39(0.03) &
38.67 \\
935 & 991(64) & 876(50) & 785(40) & 41.63(0.04) & 41.52(0.04) & 41.43(0.04) &
38.52
\enddata

